Assessing the Impact of Context Inference Error and Partial Observability on RL Methods for Just-In-Time Adaptive Interventions

Just-in-Time Adaptive Interventions (JITAIs) are a class of personalized health interventions developed within the behavioral science community. JITAIs aim to provide the right type and amount of support by iteratively selecting a sequence of intervention options from a pre-defined set of components in response to each individual's time varying state. In this work, we explore the application of reinforcement learning methods to the problem of learning intervention option selection policies. We study the effect of context inference error and partial observability on the ability to learn effective policies. Our results show that the propagation of uncertainty from context inferences is critical to improving intervention efficacy as context uncertainty increases, while policy gradient algorithms can provide remarkable robustness to partially observed behavioral state information.

==> pictures/methods/conclusions.tex <==
\section{Conclusions}\label{sec:conclusions}

In this paper we have investigated the impact of context inference error and partial observability on the ability to learn intervention option selection policies for Just-In-Time adaptive interventions using RL methods. We have introduced a novel simulation environments that captures key aspects of JITAIs including habituation and disengagement risk as well as uncertainty and error in context inferences. We have investigated learning policies which rely on most likely inferred context (as is typically the case in current JITAIs), and have shown that the use of context probabilities significantly outperforms the use of most likely context inferences. We have further shown that there is a stark difference in performance between policy gradient methods and Q-learning methods under partial observability. 

As noted in Section \ref{subsec:rl-jitais} this work has a number of important limitations. First, our primary goal is to quantify the fundamental limits of policy learnability under context inference error and uncertainty as well as partial observability using policy gradient and Q-learning methods. In doing so we have not constrained the RL methods to a realistic number of episodes during learning. As a result, our findings should be interpreted as providing upper bounds on performance in these important and previously unexplored settings. 

Going forward, more work is required to compose the findings of this paper with regard to the use of probabilistic context inference representations with prior work such as \cite{liao2020personalized}, which focuses on sample efficiency of learning. We also note that the drastic loss of performance experienced by traditional Q-learning methods in our experiments may be addressable using state augmentation methods such as the addition of memory or the use of recurrent neural networks that have been proposed in prior work to deal with partial observability. Another potentially interesting possibility is the incorporation of probabilistic dynamic latent variable models to provide beliefs over the full state including psychological latent variables.  

Finally, we note that while the simulation environment was designed to model key issues with context uncertainty and delayed effect of actions, it is limited in other aspects. Nevertheless we believe that the insights we derive have important implications for the development of RL methods that can be applied to improve the effectiveness of real-world JITAIs.



